Enabling certification of verification-agnostic networks via memory-efficient semidefinite programming

Convex relaxations have emerged as a promising approach for verifying desirable properties of neural networks like robustness to adversarial perturbations. Widely used Linear Programming (LP) relaxations only work well when networks are trained to facilitate verification. This precludes applications that involve verification-agnostic networks, i.e., networks not specially trained for verification. On the other hand, semidefinite programming (SDP) relaxations have successfully be applied to verification-agnostic networks, but do not currently scale beyond small networks due to poor time and space asymptotics. In this work, we propose a first-order dual SDP algorithm that (1) requires memory only linear in the total number of network activations, (2) only requires a fixed number of forward/backward passes through the network per iteration. By exploiting iterative eigenvector methods, we express all solver operations in terms of forward and backward passes through the network, enabling efficient use of hardware like GPUs/TPUs. For two verification-agnostic networks on MNIST and CIFAR-10, we significantly improve L-inf verified robust accuracy from 1% to 88% and 6% to 40% respectively. We also demonstrate tight verification of a quadratic stability specification for the decoder of a variational autoencoder.

==> app-fast-prox.tex <==
\subsection{Initialization via fast dual proximal method}\label{app:fast-prox}
Suppose we have an objective of the form 
\begin{align}
    u(\lambda) + v\br{\mathcal{A}\br{\lambda}}\label{eq:dual_prox}
\end{align}
where $\mathcal{A}$ is a linear operator and $u, v$ are convex functions with $u$ being differentiable and $v$ being prox-friendly (ie we can compute the prox operator of $v$ efficiently). The fast dual proximal gradient method \cite{beck2014fast} applies to optimization problems of this form, but requires $u$ to be strongly convex in addition. 
We can achieve this by simply adding a term of the form ${\norm{\lambda-\lambda^t}}^2$ to $u$ where $\lambda^t$ is an arbitrary  ``guess'' for the dual variables. We can solve the problem to some accuracy with a fixed choice of $\lambda^0$ and then set $\lambda^1$ to the resulting optimal value. Thus in turn is simply the proximal gradient method applied to \eqref{eq:dual_prox}, with each proximal step being solved using an inner loop that involves applying the fast dual proximal gradient method to the objective function
\[u(\lambda) + \frac{1}{2\eta}{\norm{\lambda-\lambda^t}}^2+ v\br{\mathcal{A}\br{\lambda}}\]


